A Noise-Tolerant Quasi-Newton Algorithm for Unconstrained Optimization

This paper describes an extension of the BFGS and L-BFGS methods for the minimization of a nonlinear function subject to errors. This work is motivated by applications that contain computational noise, employ low-precision arithmetic, or are subject to statistical noise. The classical BFGS and L-BFGS methods can fail in such circumstances because the updating procedure can be corrupted and the line search can behave erratically. The proposed method addresses these difficulties and ensures that the BFGS update is stable by employing a lengthening procedure that spaces out the points at which gradient differences are collected. A new line search, designed to tolerate errors, guarantees that the Armijo-Wolfe conditions are satisfied under most reasonable conditions, and works in conjunction with the lengthening procedure. The proposed methods are shown to enjoy convergence guarantees for strongly convex functions. Detailed implementations of the methods are presented, together with encouraging numerical results.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk --shell-escape -pdf \"$_[0]\"" );
    }
}

==> old_material.tex <==
\section{Old Material}

We propose multiple conditions for lengthening the curvature pairs. For clarity, the parameter $\alpha_k$ here refers to the lengthening parameter and not the steplength. Note that all criteria would require more in-depth modification of the algorithmic procedure of the line search itself.

\subsection{Modified Wolfe Condition}

Recall that the Wolfe condition is defined as
\begin{equation*}
    p_k^T \nabla \phi(x_k + \alpha_k p_k) \geq c_2 p_k^T \nabla \phi(x_k)
\end{equation*}
which, if we define $h_k(\alpha) = \phi(x_k + \alpha p_k)$, is equivalent to
\begin{equation*}
    h^\prime(\alpha_k) \geq c_2 h^\prime(0).
\end{equation*}

Replacing the true gradient with the observed gradient, we obtain the condition
\begin{equation*}
    p_k^T g(x_k + \alpha_k p_k) \geq c_2 p_k^T g(x_k).
\end{equation*}
If we define 
\begin{equation*}
    s_k = \alpha_k p_k,\quad y_k = g(x_k + \alpha_k p_k) - g(x_k),
\end{equation*}
we have that
\begin{align*}
    p_k^T g(x_k + \alpha_k p_k) \geq c_2 p_k^T g(x_k)
    ~~~ \Leftrightarrow ~~~  s_k^T y_k \geq -(1-c_2) s_k^T g(x_k).
\end{align*}

At first glance, this might appear sufficient for ensuring that $s_k^T y_k > 0$, given that $p_k$ is a descent direction with respect to $g(x_k)$. However, in the presence of noise, it is not enough to simply ensure $s_k^T y_k > 0$, because the noise in $y_k$, $e(x_k + \alpha_k p_k) - e(x_k)$, may significantly alter the actual difference in the true gradients $\nabla \phi(x_k + \alpha_k p_k) - \nabla \phi(x_k)$, rendering the curvature information inaccurate or useless. 

In order to ensure that the difference in gradients is not dominated by noise, we propose the following conditions:
\begin{equation}
    \label{eq:modified_wolfe_cond_1}
    p_k^T g(x_k + \alpha_k p_k) \geq c_2 p_k^T g(x_k) + 2(1 + c_3) \epsilon_g \|p_k\|, \quad 0 < c_2 < 1, c_3 > 0,
\end{equation}
or alternatively, 
\begin{equation}
    \label{eq:modified_wolfe_cond_2}
    p_k^T g(x_k + \alpha_k p_k) \geq \max\{c_2 p_k^T g(x_k),~2(1 + c_3) \epsilon_g \|p_k\|\}, \quad 0 < c_2 < 1, c_3 > 0.
\end{equation}
Both of these conditions offer two benefits: (1) as $\epsilon_g \rightarrow 0$, the conditions revert to the original Wolfe condition, and (2) they guarantee that the curvature information is not dominated by noise.

In particular, note that when \eqref{eq:modified_wolfe_cond_1} holds, we have that
\begin{align*}
    p_k^T (g(x_k + \alpha_k p_k) - g(x_k)) & \geq -(1 - c_2) p_k^T g(x_k) + 2(1 + c_3)\epsilon_g \|p_k\| \\
    & \geq 2(1 + c_3)\epsilon_g \|p_k\|
\end{align*}
since $p_k^T g(x_k) \leq 0$. When \eqref{eq:modified_wolfe_cond_2} holds, we similarly have that
\begin{equation*}
    p_k^T g(x_k + \alpha_k p_k) \geq 2(1 + c_3) \epsilon_g \|p_k\|.
\end{equation*}
This implies that
\begin{align*}
    p_k^T (g(x_k + \alpha_k p_k) - g(x_k)) & \geq -p_k^T g(x_k) + 2(1 + c_3) \epsilon_g \|p_k\| \\
    & \geq 2(1 + c_3) \epsilon_g \|p_k\|.
\end{align*}
Under both \eqref{eq:modified_wolfe_cond_1} and \eqref{eq:modified_wolfe_cond_2}, we obtain
\begin{equation*}
    u_k^T (g(x_k + \alpha_k p_k) - g(x_k)) \geq 2(1 + c_3) \epsilon_g
\end{equation*}
where
\begin{equation*}
    u_k = \frac{p_k}{\lVert p_k \rVert}
\end{equation*}
is the unit vector along $p_k$. 

One can show that this equation ensures the noise does not dominate the difference in gradients, i.e.,
\begin{equation*}
    u_k^T (\nabla \phi(x_k + \alpha_k p_k) - \nabla \phi(x_k)) \geq c_3 u_k^T (e(x_k + \alpha_k p_k) - e(x_k)).
\end{equation*}
We formalize this in Theorem \ref{thm:curvature}.

\begin{theorem} \label{thm:curvature}
Suppose $\alpha_k$ satisfies
\begin{equation}
    \label{eq:modified_wolfe_cond}
    p_k^T (g(x_k + \alpha_k p_k) - g(x_k)) \geq 2(1 + c_3) \epsilon_g \lVert p_k \rVert
\end{equation}
Then we have 
\begin{equation*}
    p_k^T (\nabla \phi(x_k + \alpha_kp_k) - \nabla \phi(x_k)) \geq 2 c_3 \epsilon_g \lVert p_k \rVert \geq c_3 p_k^T (e(x_k + \alpha_k p_k) - e(x_k))
\end{equation*}
which implies that
\begin{equation*}
  \left(1 - \frac{1}{c_3} \right) s_k^T \widetilde y_k \leq s_k^T y_k \leq \left(1 + \frac{1}{c_3} \right) s_k^T \widetilde y_k
\end{equation*}
where
\begin{align*}
    y_k & = g(x_k + \alpha_k p_k) - g(x_k) \\
    \widetilde y_k & = \nabla \phi(x_{k} + \alpha_k p_k) - \nabla \phi(x_k)
\end{align*}
Hence we can obtain \textbf{accurate} curvature information by using $(s_k, y_k)$ in place of $(s_k, \widetilde y_k)$.
\end{theorem}

\begin{proof}
To see the first set of inequalities, recall that $g(x) = \nabla \phi(x) + e(x)$ and $\|e(x)\| \leq \epsilon_g$ for all $x \in \mathbb{R}^d$. Hence, \eqref{eq:modified_wolfe_cond} implies that
\begin{align*}
    p_k^T (\nabla \phi(x_k + \alpha_k p_k) - \nabla \phi(x_k)) & \geq 2(1 + c_3) \epsilon_g \|p_k\| - p_k^T (e(x_k + \alpha_k p_k) - e(x_k)) \\
    & \geq 2 (1 + c_3) \epsilon_g \|p_k\| - \|p_k\|(\| e(x_k + \alpha_k p_k) \| + \|e(x_k)\|) \\
    & \geq 2 (1 + c_3) \epsilon_g \|p_k\| - 2 \epsilon_g \|p_k\| \\
    & = 2 c_3 \epsilon_g \|p_k\|.
\end{align*}
To see the other inequality, note that
\begin{align*}
    c_3 p_k^T (e(x_k + \alpha_k p_k) - e(x_k)) & \leq c_3 \|p_k\| (\|e(x_k + \alpha_k p_k)\| + \|e(x_k)\|) \\
    & = 2 c_3 \epsilon_g \|p_k\|.
\end{align*}
Using these inequalities, we can therefore show that
\begin{align*}
    s_k^T y_k & = \alpha_k p_k^T (g(x_k + \alpha_k p_k) - g(x_k)) \\
    & = \alpha_k p_k^T (\nabla \phi(x_k + \alpha_k p_k) - \nabla \phi(x_k)) + \alpha_k p_k^T (e(x_k + \alpha_k p_k) - e(x_k)) \\
    & \leq \alpha_k \left(1 + \frac{1}{c_3} \right) p_k^T (\nabla \phi(x_k + \alpha_k p_k) - \nabla \phi(x_k)) \\
    & = \left( 1 + \frac{1}{c_3} \right) s_k^T \tilde{y}_k.
\end{align*}
Similarly, 
\begin{align*}
    s_k^T y_k & = \alpha_k p_k^T (g(x_k + \alpha_k p_k) - g(x_k)) \\
    & = \alpha_k p_k^T (\nabla \phi(x_k + \alpha_k p_k) - \nabla \phi(x_k)) + \alpha_k p_k^T (e(x_k + \alpha_k p_k) - e(x_k)) \\
    & \geq \alpha_k \left(1 - \frac{1}{c_3} \right) p_k^T (\nabla \phi(x_k + \alpha_k p_k) - \nabla \phi(x_k)) \\
    & = \left( 1 - \frac{1}{c_3} \right) s_k^T \tilde{y}_k
\end{align*}
as desired.
\end{proof}


As a sanity check, consider the case of strongly convex function. If $\phi(\cdot)$ is $m$-strongly convex, then we naturally have
\begin{equation*}
     p_k^T (\nabla \phi(x_k + \alpha_k p_k) - \nabla \phi(x_k)) \geq m \alpha_k \lVert p_k\rVert^2.
\end{equation*}
To ensure that we have \eqref{eq:modified_wolfe_cond}, we need to ensure that
\begin{equation*}
    m \alpha_k \lVert p_k\rVert^2 - 2 \epsilon_g \lVert p_k\rVert \geq 2 (1 + c_3) \epsilon_g \lVert p_k\rVert
\end{equation*}
i.e.,
\begin{equation*}
    m \alpha_k \lVert p_k\rVert \geq 2 (2 + c_3) \epsilon_g 
\end{equation*}
or
\begin{equation*}
    \lVert s_k \rVert \geq 2(2 + c_3)\frac{\epsilon_g}{m}
\end{equation*}
which is very similar to the requirement of the lengthening parameter. 

Now, note that not all functions $\phi(\cdot)$ can ensure the existence of a stepsize that satisfies \eqref{eq:modified_wolfe_cond}. Therefore we make the following assumption:
\begin{equation}
    \label{eq:unbounded_directional_derivative}
    \lim_{\alpha \to + \infty}~p^T \nabla \phi(x + \alpha p) = +\infty,\quad \forall x, p \in \mathbb{R}^d
\end{equation}
or equivalently,
\begin{equation*}
    \lim_{\alpha \to  +\infty}~h_{x,p}^\prime(\alpha) = +\infty, \quad \forall x, p \in \mathbb{R}^d
\end{equation*}
where $h_{x, p}(\alpha) = \phi(x + \alpha p)$. This means that the function $\phi(\cdot)$, while allowed to be non-convex, must ``behave like'' a strongly convex function asymptotically. This requirement is intuitively obvious, since a function that becomes asymptotically flat cannot provide useful curvature information to build a convex quadratic interpolating model, which is required by BFGS method. 

It is also obvious that if $\phi(\cdot)$ satisfies \eqref{eq:unbounded_directional_derivative}, then for sufficiently large $\alpha_k$, \eqref{eq:modified_wolfe_cond} will always be satisfied. 

\subsection{Modified Lengthening Condition}

Whereas [BFGSwErrorsPaper] requires knowledge of the strong convexity parameter, one can instead use a local estimate of the curvature of the function along the direction $s_k$. This yields the proposed condition
\begin{equation}
    \|s_k\| \geq l ~~~~~~~\mbox{where } l > \frac{2 \epsilon_g}{\hat{m}} \mbox{ and } \hat{m} = \frac{y_k^T s_k}{s_k^T s_k}.
\end{equation}
One can show that this criterion guarantees that $\frac{y_k^T s_k}{s_k^T s_k}$ will be lower bounded (as needed in the [ToolPaper]), but yields a more pessimistic upper bound.

\subsection{Noise Robustness Condition}

An alternative to the first two conditions (which modify the Wolfe condition) is to consider the additional condition

\subsection{Natural Steplength Estimation}

In the deterministic setting, the unit steplength is considered the ``natural'' steplength for BFGS because it is guaranteed to be accepted for sufficient large $k$ and permits superlinear convergence to the solution. To see this, recall that Taylor's theorem gives
\begin{equation}
    \phi(x_k + \alpha_k p_k) = \phi(x_k) + \alpha_k \nabla \phi(x_k)^T p_k + \frac{1}{2} \alpha_k^2 p_k^T \nabla^2 \phi(x_k) p_k + O(\|p_k\|^3).
\end{equation}
Assuming $H_k \approx \nabla^2 \phi(x_k)^{-1}$ (although a weaker condition is permissible; see \cite{nocedal2006numerical}), one can intuit that when one is sufficiently close to the solution (i.e. $\|p_k\|$ is sufficiently small), we have that for $\alpha_k = 1$,
\begin{align}
    \phi(x_k +\alpha_k p_k) & \approx \phi(x_k) - \alpha_k \nabla \phi(x_k)^T H_k \nabla \phi(x_k) + \frac{1}{2}\alpha_k^2 p_k^T H_k p_k \\
    & \approx \phi(x_k) - \alpha_k (1 - \frac{\alpha_k}{2}) \nabla \phi(x_k)^T H_k \nabla \phi(x_k).
\end{align}
Minimizing the right hand side yields $\alpha_k = 1$. Plugging this in, one can see that the Armijo condition \eqref{eq:armijo} will be satisfied with $c_1 \leq \frac{1}{2}$.

However, when entering the noisy regime, the unit steplength is no longer ``natural'' for (L-)BFGS. Assume that $g$ is a stochastic approximation to $\nabla \phi$ that is unbiased, i.e. $\mathbb{E}[g(x_k)] = \nabla \phi(x_k)$. For simplicity, assume that there is no noise in the function evaluation $\epsilon_f = 0$. Then
\begin{equation}
    \phi(x_k + \alpha_k p_k) \approx \phi(x_k) - \alpha_k \nabla \phi(x_k)^T H_k g(x_k) + \frac{1}{2} \alpha_k^2 g(x_k)^T H_k g(x_k)
\end{equation}
Taking the expectation yields
\begin{align*}
    \mathbb{E}[& \phi(x_k + \alpha_k p_k)] \\
    & \approx \phi(x_k) - \alpha_k \nabla \phi(x_k) H_k \nabla \phi(x_k) + \frac{1}{2} \alpha_k^2 \mathbb{E}[g(x_k)^T H_k g(x_k)] \\
    & \approx \phi(x_k) - \alpha_k \nabla \phi(x_k)^T H_k \nabla \phi(x_k) + \frac{\alpha_k^2}{2} \nabla \phi(x_k)^T H_k \nabla \phi(x_k) + \\ & ~~~~~~~~~~~ \frac{\alpha_k^2}{2} \mathbb{E}[(g(x_k) - \nabla \phi(x_k))^T H_k (g(x_k) - \nabla \phi(x_k))] \\
    & \approx \phi(x_k) - \alpha_k (1 - \frac{\alpha_k}{2}) \nabla \phi(x_k)^T H_k \nabla \phi(x_k) + \frac{\alpha_k^2}{2} \mathbb{E}[\|g(x_k) - \nabla \phi(x_k)\|_{H_k}^2] \\
    & \approx \phi(x_k) - \alpha_k (1 - \frac{\alpha_k}{2}) \nabla \phi(x_k)^T H_k \nabla \phi(x_k) + \\ & ~~~~~~~~~~~ \frac{\alpha_k^2}{2} \frac{\Var_{H_k}(g(x_k))}{\nabla \phi(x_k)^T H_k \nabla \phi(x_k)} \nabla \phi(x_k)^T H_k \nabla \phi(x_k) \\
    & \approx \phi(x_k) - \alpha_k \left(1 - \frac{\alpha_k}{2} \left(1 + \frac{\Var_{H_k} (g(x_k))}{\nabla \phi(x_k)^T H_k \nabla \phi(x_k)} \right) \right) \nabla \phi(x_k)^T H_k \nabla \phi(x_k)
\end{align*}
where
\begin{equation*}
    \Var_{H_k}(g(x_k)) = \mathbb{E}[\|g(x_k) - \nabla \phi(x_k)\|_{H_k}^2].
\end{equation*}
Optimizing for $\alpha_k$, we obtain
\begin{equation}
    \alpha^* = \left(1 + \frac{\Var_{H_k} (g(x_k))}{\nabla \phi(x_k)^T H_k \nabla \phi(x_k)} \right)^{-1}.
\end{equation}
We apply two approximations to this to derive our heuristic: the first approximation ignores the $H_k$ metric; the second approximation estimates the norm of the gradient by using the current norm of the gradient and the standard deviation estimate. In particular, the first approximation modifies the metric to give
\begin{equation}
    \hat{\alpha} = \left(1 + \frac{\Var (g(x_k))}{\|\nabla \phi(x_k)\|_2^2} \right)^{-1}
\end{equation}
where 
\begin{equation*}
    \Var(g(x_k)) = \mathbb{E}[\|g(x_k) - \nabla \phi(x_k)\|^2].
\end{equation*}
The second approximation estimates $\|\nabla \phi(x)\| \approx \|g(x)\|_2 - \epsilon_g$. Note, however, that this can yield a negative estimate of the norm. In order to prevent this, we safeguard the method and add a small tolerance in the denominator (which may be related to our desired gradient tolerance) to yield
\begin{equation}
    \tilde{\alpha} = \left(1 + \frac{\epsilon_g^2}{\max\{\|g(x_k)\|_2 - \epsilon_g, 0\}^2 + \epsilon_{\text{tol}^2}} \right)^{-1}.
\end{equation}
In order to enforce the use of the unit steplength in the non-noisy regime, we will revert to using the unit steplength if the predicted step is large, that is,
\begin{equation}
    \bar{\alpha} = 
    \begin{cases}
        1 & \mbox{ if } \tilde{\alpha} > \frac{1}{2} \\
        \tilde{\alpha} & \mbox{ otherwise.}
    \end{cases}
\end{equation}

% \subsubsection{Using Historical Information for Lengthening Parameter}

% The second heuristic uses historical information regarding the lengthening parameter $\beta_k$ to determine an appropriate lengthening parameter to re-initialize to when entering split phase. The heuristic is based on the observation that if the true function $\phi$ has $L$-Lipschitz continuous gradient, we have that 
% \begin{align*}
% \|g(x_k + \beta_k p_k) - g(x_k)\|_2 & = \|\nabla \phi(x_k + \beta_k p_k) - \nabla \phi(x_k) + e(x_k + \beta_k p_k) - e(x_k)\|_2 \\
% & \leq \|\nabla \phi(x_k + \beta_k p_k) - \nabla \phi(x_k)\|_2 + \|e(x_k + \beta_k p_k) - e(x_k)\|_2 \\
% & \leq L \|x_k + \beta_k p_k - x_k\|_2 + \|e(x_k + \beta_k p_k)\|_2 + \|e(x_k)\|_2 \\
% & \leq L \beta_k \|p_k\|_2 + 2 \epsilon_g.
% \end{align*}
% Since we want to ensure that
% $$\|g(x_k + \beta_k p_k) - g(x_k)\|_2 \geq 2(1 + c_3) \|p_k\|_2,$$
% we obtain that
% $$\beta_k \geq \frac{2 c_3 \epsilon_g}{L \|p_k\|_2} = C \frac{\epsilon_g}{\|p_k\|_2},$$
% where $C = \frac{2 c_3}{L}$. This corresponds to what we observe in practice, as $\beta_k$ tends to gradually increase and eventually stabilize. 

% In order to leverage this observation, we propose using historical information to provide a conservative estimate of the constant $C$. In particular, we will store a window of the last $N_{\text{window}}$ constants $C_k$ when split phase was triggered, where the constant $C_k$ is computed by
% \begin{equation}
%     C_k = \beta_k \frac{\|p_k\|_2}{\epsilon_g}.
% \end{equation}
% Denote the set of the last $N_{\text{window}}$ iterations when the  split phase was triggered as $\mathcal{K}$. If the split phase is triggered and the first heuristic using observed values from the initial phase does not work, then we will use
% \begin{equation}
%     \beta_k = \frac{\epsilon_g}{\|p_k\|_2} \min_{k \in \mathcal{K}} C_k.
% \end{equation}
% We find that this heuristic is able to eliminate many intermediate gradient evaluations at each iteration, reducing the total number of gradient evaluations significantly.

% \subsection{ECNoise for Gradient Noise Estimation}

% The design of our algorithm relies on accurate bounds on the noise, i.e.,
% \begin{equation}
%     \begin{aligned}
%         |\epsilon (x)| & \leq \epsilon_f \\
%         \|e(x)\|_2 & \leq \epsilon_g.
%     \end{aligned}
% \end{equation}
% In many cases, however, the noise level of both the function value and gradient are unknown to the user. It is hence necessary to estimate the noise. Since the noise could be deterministic or stochastic, we need a procedure for estimating the noise level in either setting. 

% Motivated by this problem, More and Wild \cite{more2011estimating} proposed a mild adaptation of Hamming's procedure \cite{hamming2012introduction} called ECNoise for estimating the noise level of a function. In particular, under a stochastic model of noise, that is, $\epsilon(x)$ is a random variable, their procedure estimates
% \begin{equation}
%     \sigma_f = ( \Var\{ \epsilon(x)\} )^{1/2}
% \end{equation}
% where $\Var\{ \epsilon(x) \}$ is the variance of the noise function. 

% Assume that the noise is unbiased, i.e. $\mathbb{E}[f(x)] = \phi(x)$. In order to convert this to an upper bound, More and Wild \cite{more2011estimating} noted that by Chebyshev's inequality, one has
% \begin{equation}
%     \mathbb{P}(|f(x) - \phi(x)| \leq \gamma \sigma_f) \geq 1 - \frac{1}{\gamma^2}.
% \end{equation}
% Thus, we can guarantee that
% \begin{equation}
%     |f(x) - \phi(x)| = |\epsilon(x)| \leq \gamma \sigma_f
% \end{equation}
% with probability at least $1 - \frac{1}{\gamma^2}$.

% In order to perform this estimation, one must assume that the noise is identically distributed in an open ball around $x$, although this may not necessarily be true in practice. Their procedure, ECNoise, samples a direction $d$ and considers the one-dimensional function at $f_d(t) = f(x + t d)$. To estimate the noise along this one-dimensional function, $f_d$ is evaluated at $t_i = t + ih$ for $i = 0, ..., m$. Let $\epsilon_d(t) = \epsilon(x + t d)$. The $k$th-order difference of this function is computed by $\Delta^0 f = f$ and
% \begin{equation}
%     \Delta^{k + 1} f_d(t) = \Delta^k[\Delta f_d(t)] = \Delta^k f_d(t + h) - \Delta^k f_d(t), ~~~ k \geq 0.
% \end{equation}
% The key relationship (proved in \cite{more2011estimating}) is given below in Theorem \ref{thm:hamming}.
% \begin{theorem}
% \label{thm:hamming}
% If the random variables $\{\epsilon(t) : t \in I\}$ are iid and if $\phi$ is continuous at $t$, then
% \begin{equation}
%     \lim_{h \rightarrow 0} \gamma_k \mathbb{E}[\Delta^k f_d (t)^2] = \sigma_f^2,
% \end{equation}
% where $\gamma_k = \frac{(k!)^2}{(2k)!}$.
% \end{theorem}
% The ECNoise method makes a particular choice of $k$ and a test for determining when the sampling distance $h$ is sufficiently small. Although this is developed under a stochastic model of noise, More and Wild \cite{more2011estimating} showed its practical applicability to both stochastic and deterministic noise.

% In order to extend the ECNoise method to bounding the norm of the gradient, we will apply ECNoise to $\|g_d(t)\|$, where $d$ is a sampled direction and $g_d(t) = g(x + td)$ is the gradient along the direction $d$. We will similarly assume that $e(x)$ is a random variable, and let $\Sigma(x) = \mathbb{E}[e(x) e(x)^T]$ denote the covariance matrix of the gradient noise. Then we define
% \begin{equation}
%     \sigma_g = \left( \sum_{i = 1}^n \Var\{ e(x)_i \} \right)^{1/2} = \sqrt{\Tr(\Sigma(x))}.
% \end{equation}
% Using this notation, we can extend Theorem \ref{thm:hamming} to the gradient case.

% \begin{corollary}
% If the random variables $\{e(t) : t \in I\}$ are iid and if $\nabla \phi$ is continuous at $t$, then
% \begin{equation}
%     \lim_{h \rightarrow 0} \gamma_k \mathbb{E}[\Delta^k \|g_d(t)\|^2] = \sigma_g^2,
% \end{equation}
% where $\gamma_k = \frac{(k!)^2}{(2k)!}$.
% \end{corollary}

% \begin{proof}
% Note that
% \begin{align*}
%     \mathbb{E}[\Delta^k \|g_d(t)\|^2] & = \mathbb{E}\left[\Delta^k \left( \sum_{i = 1}^n g_d(t)_i^2 \right) \right]\\
%     & = \mathbb{E}\left[ \sum_{i = 1}^n \Delta^k g_d(t)_i^2 \right] \\
%     & = \sum_{i = 1}^n \mathbb{E}[\Delta^k g_d(t)_i^2] \\
%     & = \sum_{i = 1}^n [ \Delta^k\{\nabla \phi(x + td)_i^2\} + \Var\{\Delta^k e(x + td)_i\}]
% \end{align*}
% where the second equality follows because the $k$th-order difference of sums is the sum of $k$th-order differences and the third equality follows from linearity of expectation. Then
% \begin{equation*}
%     \gamma_k \mathbb{E}[\Delta^k \|g_d(t)\|^2] = \gamma_k \sum_{i = 1}^n \Delta^k \{\nabla \phi(x + td)_i^2\} + \gamma_k \sum_{i = 1}^n \Var\{\Delta^k e(x + td)_i\}.
% \end{equation*}
% Taking $h \rightarrow 0$, by continuity of $\nabla \phi$, we have that $\Delta^k \{\nabla \phi(x + td)_i^2\} \rightarrow 0$, and hence the first term goes to 0. Thus,
% \begin{equation*}
%     \lim_{h \rightarrow 0} \gamma_k \mathbb{E}[\Delta^k \|g_d(t)\|^2] = \gamma_k \sum_{i = 1}^n \Var\{\Delta^k e(x + td)_i \} = \sum_{i = 1}^n \Var\{e(x + td)_i\}
% \end{equation*}
% by Theorem 2.2 in \cite{more2011estimating} applied to each component, as desired.
% \end{proof}

% Applying 


\subsection{Experiments with Only Gradient Noise}  \label{onlyg}

In this first set of experiments, the gradient contains noise but the function does not, i.e., $\epsilon_g > 0$ and $\epsilon_f = 0$. This allows us to test the efficiency of the lengthening procedure in a benign setting that avoids the effects of the noisy line search. In these experiments, all algorithms were run for a fixed number of iterations.

\subsubsection{Revisiting the \texttt{ARWHEAD} Problem}\label{revisit}

We begin by revisiting the \texttt{ARWHEAD} problem from Figure \ref{fig:BFGS on noisy ARWHEAD}, where noise was inserted with $\xi_f = 0$ and $\xi_g = 10^{-3}$. The condition number of the BFGS and BFGS-E matrices is compared in Figure \ref{fig:BFGS-E on noisy ARWHEAD}, 
and shows that the noise control condition \eqref{eq:noise} stabilizes the quasi-Newton update. 
\begin{figure}[htp]
    \centering
    % \includegraphics[width=0.4\linewidth]{plots/cond_number/norm_gks_iters_ARWHEAD_SUA_0_1e-3_1226.pdf}
    \includegraphics[width=0.49\linewidth]{final_plots/cond_number/kappa_Hs_iters_ARWHEAD_SUA_0_1e-3_1226.pdf}
    \includegraphics[width=0.49\linewidth]{final_plots/cond_number/eigvals_iters_ARWHEAD_SUA_0_1e-3_1226.pdf}
    \caption{The condition number of the BFGS and BFGS-E matrices $\kappa(H_k)$ against the number of iterations (left) and the smallest and largest eigenvalues of $B_k$ against the number of iterations (right) on the \texttt{ARWHEAD} problem.}
    \label{fig:BFGS-E on noisy ARWHEAD}
\end{figure}
It may seem surprising that in  Figure \ref{fig:BFGS-E on noisy ARWHEAD} the condition number of the BFGS matrix, $\kappa(H_k)$, decreases after having increased sharply. This can be explained by noting that as the iterates enter into the noisy regime, the difference in the gradient $y_k$ can be corrupted by noise, and we may have $s_k^T y_k \gg s_k^T \tilde{y}_k$. Thus, some of the eigenvalues of the BFGS matrix $B_k = H_k^{-1}$ will increase.  As the iteration proceeds, the rest of the eigenvalues become large too, hence decreasing the condition number.

Figure \ref{fig:obj for ARWHEAD} plots the optimality gap $\phi(x) - \phi^*$ vs the number of gradient evaluations performed for the four methods on the \texttt{ARWHEAD} problem. BFGS and L-BFGS do not achieve as high accuracy in the solution as their noise-tolerant counterparts because the deterioration in the Hessian approximation leads, at some point, to the generation of very small steps that severely limit the decrease in the objective function. The behavior of the methods on this problem is typical of what we have observed. In particular BFGS-E and L-BFGS-E  trigger lengthening of the curvature pairs prior to the point where BFGS and L-BFGS stagnate due to noise. This indicates that the lengthening procedure stabilizes the Hessian approximation prior to reaching this neighborhood.


\begin{figure}[htp]
    \centering
    \includegraphics[width=0.32\linewidth]{final_plots/grad_noise/BFGS/obj_ts_grad_evals_ARWHEAD_SUA_0_1e-1_1226.pdf}
    \includegraphics[width=0.32\linewidth]{final_plots/grad_noise/BFGS/obj_ts_grad_evals_ARWHEAD_SUA_0_1e-3_1226.pdf}
    \includegraphics[width=0.32\linewidth]{final_plots/grad_noise/BFGS/obj_ts_grad_evals_ARWHEAD_SUA_0_1e-5_1226.pdf}
    \includegraphics[width=0.32\linewidth]{final_plots/grad_noise/L-BFGS/obj_ts_grad_evals_ARWHEAD_SUA_0_1e-1_1226.pdf}
    \includegraphics[width=0.32\linewidth]{final_plots/grad_noise/L-BFGS/obj_ts_grad_evals_ARWHEAD_SUA_0_1e-3_1226.pdf}
    \includegraphics[width=0.32\linewidth]{final_plots/grad_noise/L-BFGS/obj_ts_grad_evals_ARWHEAD_SUA_0_1e-5_1226.pdf}
    % \includegraphics[width=0.4\linewidth]{plots/grad_noise/objs_iters_ARWHEAD_SUA_0_1e-1_1226.pdf}
    % \includegraphics[width=0.4\linewidth]{plots/grad_noise/objs_iters_ARWHEAD_SUA_0_1e-3_1226.pdf}
    % \includegraphics[width=0.4\linewidth]{plots/grad_noise/objs_iters_ARWHEAD_SUA_0_1e-5_1226.pdf}
    % \includegraphics[width=0.4\linewidth]{plots/grad_noise/objs_iters_ARWHEAD_SUA_0_1e-7_1226.pdf}
    \caption{The true optimality gap $\phi(x_k) - \phi^*$ against the number of gradient evaluations on the \texttt{ARWHEAD} problem for $\epsilon_f=0$, and for the following gradient noise levels:  $\xi_g = 10^{-1}$ (left), $10^{-3}$ (middle), and $10^{-5}$ (right). The top row compares BFGS against BFGS-E and the bottom row compares L-BFGS against L-BFGS-E. The black dashed line denotes the iteration before the split phase becomes active.}
    \label{fig:obj for ARWHEAD}
\end{figure}

The lengthening procedure in our noise-tolerant algorithms comes at an additional computational cost. Figure~\ref{fig:grad evals for ARWHEAD} plots the cumulative number of gradient evaluations against the iteration count for the \texttt{ARWHEAD} problem. We observe that for BFGS or L-BFGS, the cumulative number of gradient evaluations is approximately equal to the number of iterations.
For the noise-tolerant methods, the number of gradient evaluations match the standard BFGS and L-BFGS methods until the split phase activates. Upon entering the split phase, we notice that the cost of each iteration is approximately $2-4$ gradient evaluations. This may be explained by the additional $1-3$ gradient evaluations necessary to find the appropriate $\beta_k$ that satisfies both the noise and Wolfe conditions, plus one gradient evaluation for triggering the split phase. This cost is  worthwhile in that it allows the algorithm to make progress in the noisy regime.

\begin{figure}
    \centering
    \includegraphics[width=0.32\linewidth]{final_plots/grad_noise/BFGS/grad_evals_iters_ARWHEAD_SUA_0_1e-1_1226.pdf}
    \includegraphics[width=0.32\linewidth]{final_plots/grad_noise/BFGS/grad_evals_iters_ARWHEAD_SUA_0_1e-3_1226.pdf}
    \includegraphics[width=0.32\linewidth]{final_plots/grad_noise/BFGS/grad_evals_iters_ARWHEAD_SUA_0_1e-5_1226.pdf}
    % \includegraphics[width=0.4\linewidth]{plots/grad_noise/grad_evals_iters_ARWHEAD_SUA_0_1e-1_1226.pdf}
    % \includegraphics[width=0.4\linewidth]{plots/grad_noise/grad_evals_iters_ARWHEAD_SUA_0_1e-3_1226.pdf}
    % \includegraphics[width=0.4\linewidth]{plots/grad_noise/grad_evals_iters_ARWHEAD_SUA_0_1e-5_1226.pdf}
    % \includegraphics[width=0.4\linewidth]{plots/grad_noise/grad_evals_iters_ARWHEAD_SUA_0_1e-7_1226.pdf}
    \caption{Cumulative number of gradient evaluations against the iteration count on the \texttt{ARWHEAD} problem for $\epsilon_f=0$ and gradient noise levels $\xi_g = 10^{-1}$ (left), $10^{-3}$ (middle), and $10^{-5}$ (right) for BFGS and BFGS-E. The results for L-BFGS and L-BFGS-E are similar. The black dashed line denotes the iteration before the split phase becomes active.}
    \label{fig:grad evals for ARWHEAD}
\end{figure}

% After the first few iterations of a typical BFGS or L-BFGS run, one frequently accepts the unit steplength resulting in only one additional gradient evaluation at each iteration. Therefore, one expects that the cumulative number of gradient evaluations is approximately equal to the number of iterations. In the noisy regime, this behavior mostly persists due to the presence of noise, except for problems with high noise ($\xi_g = 10^{-1}, 10^{-3}$) where the line search fails in the noisy regime while backtracking, therefore accumulating no gradient evaluations for those iterations. 

% For the noise-tolerant methods, upon entering the split phase, we notice that the cost of each iteration is approximately $2-4$ gradient evaluations. This may be explained by the additional $1-3$ gradient evaluations necessary to find the appropriate $\beta_k$ that satisfies both the noise and Wolfe conditions, plus one gradient evaluation for triggering the split phase. This cost is  worthwhile by the additional progress the algorithm can make under the presence of noise after stabilizing the (L-)BFGS matrix via lengthening.

% \subsubsection{Experiments with Skewed Gradient Noise} \label{sec:skewed grad}

% In our initial set of experiments, we assumed that the gradient noise is distributed equally across all components such that $\xi_g^i = \xi_g$ for all $i$. This will therefore always introduce noise into the gradient regardless of its direction. Instead of evenly distributing the noise across all components, we can instead consider anisotropic noise where only a fraction $f$ of the components are contaminated with noise, restricting noisy directions to a small subspace. 

% If we call this set of selected random indices $I$, then for $\xi_g \in \{10^{-1}, 10^{-3}, 10^{-5}, 10^{-7}\}$ and $f \in \{0.1, 0.5, 0.9\}$, we will choose
% \begin{equation}
%     \xi_g^i = 
%     \begin{cases}
%         \frac{1}{\sqrt{f}} \xi_g & \mbox{ if } i \in I \\
%         0 & \mbox{ otherwise.}
%     \end{cases}
% \end{equation}
% Dividing by $\sqrt{f}$ ensures that $\|e(x)\|^2 \leq \sum_{i = 1}^d (\xi_g^i)^2 = \frac{1}{f} \sum_{i = 1}^{fd} \xi_g^2 = d \xi_g^2$, so $\|e(x)\| \leq \sqrt{d} \xi_g$, which is consistent with our noise level from before. Notice that $I$ is fixed over the entire run.

% For easier problems, such as problems where the objective function does not have degenerate curvature near the solution or is not highly nonlinear, we observe similar results to what we have seen in prior examples. However, for a handful of problems, we can observe instances where lengthening for the skewed problem hurts the iteration. This is depicted through the \texttt{BDQRTIC} example in Figure \ref{fig:BDQRTIC skewed}.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.4\textwidth]{{plots/skewed/objs_iters_BDQRTIC_SUAK_0.1_0_1e-1_1226}.pdf}
%     \includegraphics[width=0.4\textwidth]{{plots/skewed/objs_iters_BDQRTIC_SUAK_0.5_0_1e-1_1226}.pdf}
%     \includegraphics[width=0.4\textwidth]{{plots/skewed/objs_iters_BDQRTIC_SUAK_0.9_0_1e-1_1226}.pdf}
%     \caption{The objective function $f(x_k) - f^*$ against the number of iterations on the \texttt{BDQRTIC} problem with skewed noise for noise level $\xi_g = 10^{-1}$ and fraction $f = 0.1$ (top left), $0.5$ (top right), and $0.9$ (bottom).}
%     \label{fig:BDQRTIC skewed}
% \end{figure}

% To explain the discrepancy in performance, note that when $f$ is small, noise only influences a small percentage of the components of the gradient. Therefore, if the given noise level $\epsilon_g$ is high but the majority of the search directions do not encounter noise, the lengthening procedure, by enforcing the right hand side of the noise condition as $\epsilon_g \|p_k\|$, is too strong, generating non-local curvature information unnecessarily while standard methods can benefit from more local curvature along non-noisy directions. These experiments suggest that if one had the capability to estimate the noise along a particular direction, then one could instead use information about the noise along a specific direction, such as \eqref{eq:direct noise cond}. Since uncertainty quantification methods of this kind lie outside of the scope of this paper, we leave this work for future research.

\subsubsection{Comparison to Skipping}\label{skip}

It was mentioned in \S\ref{motivation} that one possible approach for handling noise is to skip the BFGS update when the noise control condition is not satisfied for $c_3 = 0$, that is,
\begin{equation}
    (g(x_k + \alpha_k p_k) - g(x_k))^T p_k < 2 \epsilon_g \|p_k\|.
\end{equation}
We have experimentally found that skipping, if done properly, can be a strong alternative to lengthening if the problem is fairly well-conditioned and the Hessian does not change much, using much fewer gradient evaluations than the two-phase line search. However, it can fail to capture the change in curvature that is necessary for more difficult problems. This is demonstrated in the \texttt{EIGENCLS} example in Figure \ref{fig:obj for EIGENCLS}. Continuing to update the BFGS matrix using lengthening is able to continue to improve the quality of the Hessian approximation, leading to faster decrease in the objective value compared to skipping.

\begin{figure}[htp]
    \centering
    \includegraphics[width=0.32\linewidth]{final_plots/grad_noise/BFGS/obj_ts_grad_evals_EIGENCLS_SUA_0_1e-1_1226.pdf}
    \includegraphics[width=0.32\linewidth]{final_plots/grad_noise/BFGS/obj_ts_grad_evals_EIGENCLS_SUA_0_1e-3_1226.pdf}
    \includegraphics[width=0.32\linewidth]{final_plots/grad_noise/BFGS/obj_ts_grad_evals_EIGENCLS_SUA_0_1e-5_1226.pdf}
    \includegraphics[width=0.32\linewidth]{final_plots/grad_noise/L-BFGS/obj_ts_grad_evals_EIGENCLS_SUA_0_1e-1_1226.pdf}
    \includegraphics[width=0.32\linewidth]{final_plots/grad_noise/L-BFGS/obj_ts_grad_evals_EIGENCLS_SUA_0_1e-3_1226.pdf}
    \includegraphics[width=0.32\linewidth]{final_plots/grad_noise/L-BFGS/obj_ts_grad_evals_EIGENCLS_SUA_0_1e-5_1226.pdf}
    % \includegraphics[width=0.4\linewidth]{plots/grad_noise/objs_iters_EIGENCLS_SUA_0_1e-1_1226.pdf}
    % \includegraphics[width=0.4\linewidth]{plots/grad_noise/objs_iters_EIGENCLS_SUA_0_1e-3_1226.pdf}
    % \includegraphics[width=0.4\linewidth]{plots/grad_noise/objs_iters_EIGENCLS_SUA_0_1e-5_1226.pdf}
    % \includegraphics[width=0.4\linewidth]{plots/grad_noise/objs_iters_EIGENCLS_SUA_0_1e-7_1226.pdf}
    \caption{The true optimality gap $\phi(x_k) - \phi^*$ against the number of gradient evaluations on the \texttt{EIGENCLS} problem for $\epsilon_f=0$, and for the following gradient noise levels:  $\xi_g = 10^{-1}$ (left), $10^{-3}$ (middle), and $10^{-5}$ (right). The top row compares BFGS, BFGS with skipping, and BFGS-E and the bottom row compares L-BFGS, L-BFGS with skipping, and L-BFGS-E. The black dashed line denotes the iteration before the split phase becomes active.}
    \label{fig:obj for EIGENCLS}
\end{figure}

In addition, the noise level in the gradient evaluation may fluctuate rather than remain constant in some applications. One special case is that of intermittent noise. 
% We have already demonstrated how inserting noise into standard BFGS updating contaminates the Hessian approximation and harms the BFGS iteration. We will additionally demonstrate that once it is contaminated, the BFGS matrix cannot self-correct quickly, while our methods can almost immediately take advantage of gradient evaluations with diminished noise. 
To simulate it, we will set $\xi_f=0$ and let the noise level in the gradient $\xi_g$ alternate between 0 and a fixed nonzero value every $N_{\text{noise}}$ iterations, where $N_{\text{noise}} \in \{10, 25, 50\}$. We show representative results using the \texttt{CRAGGLVY} problem in Figure \ref{fig:intermit CRAGGLVY}. The noise-tolerant and skipping methods are provided the value of $\epsilon_g$ but not $N_{\text{noise}}$.

BFGS suffers the most from the inclusion of intermittent noise, and is unable to recover quickly enough to make progress even when there is no noise in the gradient. The skipping methods are able to make faster progress when noise is diminished but not as quickly as the noise-tolerant methods since they do not benefit from good updates to the BFGS matrix. In contrast, BFGS-E is able to continue to make progress immediately once noise is diminished; see in particular the stepwise behavior on the top right plot in Figure \ref{fig:intermit CRAGGLVY}. L-BFGS-E performs even better than BFGS-E, but note that standard L-BFGS is quite effective when the noise toggles every $N_{\text{noise}}=25$ or 50 iterations. This is because, if the number $N_{\text{noise}}$ of non-noisy iterations is larger than the memory $t = 10$, L-BFGS is able to forget all noise-contaminated curvature pairs, then it is able to recover and make progress. 

\begin{figure}[htp]
    \centering
    \includegraphics[width=0.32\linewidth]{final_plots/intermit/BFGS/obj_ts_iters_CRAGGLVY_SUAI_10_0_1e-1_1226.pdf}
    \includegraphics[width=0.32\linewidth]{final_plots/intermit/BFGS/obj_ts_iters_CRAGGLVY_SUAI_25_0_1e-1_1226.pdf}
    \includegraphics[width=0.32\linewidth]{final_plots/intermit/BFGS/obj_ts_iters_CRAGGLVY_SUAI_50_0_1e-1_1226.pdf}
    \includegraphics[width=0.32\linewidth]{final_plots/intermit/L-BFGS/obj_ts_iters_CRAGGLVY_SUAI_10_0_1e-1_1226.pdf}
    \includegraphics[width=0.32\linewidth]{final_plots/intermit/L-BFGS/obj_ts_iters_CRAGGLVY_SUAI_25_0_1e-1_1226.pdf}
    \includegraphics[width=0.32\linewidth]{final_plots/intermit/L-BFGS/obj_ts_iters_CRAGGLVY_SUAI_50_0_1e-1_1226.pdf}
    % \includegraphics[width=0.4\textwidth]{plots/intermit/objs_iters_CRAGGLVY_SUAI_10_0_1e-1_1226.pdf}
    % \includegraphics[width=0.4\textwidth]{plots/intermit/objs_iters_CRAGGLVY_SUAI_25_0_1e-1_1226.pdf} \\
    % \includegraphics[width=0.4\textwidth]{plots/intermit/objs_iters_CRAGGLVY_SUAI_50_0_1e-1_1226.pdf}
    % \includegraphics[width=0.4\textwidth]{plots/intermit/objs_iters_CRAGGLVY_SUAI_100_0_1e-1_1226.pdf} 
    \caption{Intermittent Noise. Optimality gap $\phi(x_k) - \phi^*$ against the number of iterations on the \texttt{CRAGGLVY} problem. $\xi_f=0$ and $\xi_g$ alternates between 0 and with $\xi_g = 10^{-1}$ every $N_{\text{noise}}$ iterations. Results for $N_{\text{noise}} = 10$ (left), $25$ (middle), and $50$ (right). The top row compares BFGS, BFGS with skipping, and BFGS-E and the bottom row compares L-BFGS, L-BFGS with skipping, and L-BFGS-E. The black dashed line denotes the iteration before the split phase becomes active.}
    \label{fig:intermit CRAGGLVY}
\end{figure}

Since skipping is not as robust as lengthening for handling difficult problems and adapting to fluctuating noise, we do not report its numerical results for the experiments in the following section.

